Tetra and Didi, the cosmic spectral twins

We introduce a pair of isospectral but non-isometric compact flat 3-manifolds called Tetra (a tetracosm) and Didi (a didicosm). The closed geodesics of Tetra and Didi are very different. Where Tetra has two quarter-twisting geodesics of the shortest length, Didi has four half-twisting geodesics. Nevertheless, these spaces are isospectral. This isospectrality can be proven directly by matching eigenfunctions having the same eigenvalue. However, the real interest of this pair--and what led us to discover it--is the way isospectrality emerges from the Selberg trace formula, as the result of a delicate interplay between the lengths and twists of closed geodesics.

==> cosmic_dot_bib <==
@book{weeks:sos,
	author =	"Jeffrey R. Weeks",
	title =		"The Shape of Space, Second Edition",
	publisher =	"Dekker",
	year =		"2001"
}
@book{weeks:sosmovie,
	author =	"Jeffrey R. Weeks",
	title =		"The Shape of Space (the movie)",
	publisher =	"Minnesota Geometry Center",
	year =		"1995"
}
@article{weeks:curved,
	author =	"Jeffrey R. Weeks",
	title =		"Real-time rendering in curved spaces",
	journal =	"IEEE Computer Graphics and Applications",
	volume =	"22",
        pages="90-99",
	year =		"Nov/Dec 2002"
}
@article {reid:isospec,
    AUTHOR = {Reid, Alan W.},
     TITLE = {Isospectrality and commensurability of arithmetic hyperbolic
              {$2$}- and {$3$}-manifolds},
   JOURNAL = {Duke Math. J.},
    VOLUME = {65},
      YEAR = {1992},
     PAGES = {215-228}
}
@article {gangolli:selberg,
    AUTHOR = {Gangolli, Ramesh},
     TITLE = {The length spectra of some compact manifolds of negative
              curvature},
   JOURNAL = {J. Differential Geom.},
    VOLUME = {12},
      YEAR = {1977},
    NUMBER = {3},
     PAGES = {403--424}
}
@incollection {bb:selberg,
    AUTHOR = {B{\'e}rard-Bergery, Lionel},
     TITLE = {Laplacien et g\'eod\'esiques ferm\'ees sur les formes d'espace
              hyperbolique compactes},
 BOOKTITLE = {S\'eminaire Bourbaki, 24\`eme ann\'ee (1971/1972), Exp. No.
              406},
     PAGES = {107--122. Lecture Notes in Math., Vol. 317},
 PUBLISHER = {Springer},
      YEAR = {1973}
}

@misc{conwayrossetti:hearing,
title = {{Hearing the platycosms}},
author = {Juan Pablo Rossetti and John Horton Conway},
eprint = {arXiv:math.DG/0311470}}

@misc{conwayrossetti:seeing,
title = {{Describing the platycosms}},
author = {John Horton Conway and Juan Pablo Rossetti},
eprint = {arXiv:math.DG/0311476}}

@article{doylerossetti:cosmic,
title = {{Tetra and Didi, the cosmic spectral twins}},
author = {Peter G. Doyle and Juan Pablo Rossetti},
journal = {Geom. Topol.},
volume = 8,
year = 2004,
pages = {1227--1242},
eprint = {arXiv:math.DG/0407422}}

@article{huber:selbergI,
	author =	"Heinz Huber",
	title =	"Zur analytischen {T}heorie hyperbolischer {R}aumformen und {B}ewegungsgruppen, {I}",
	journal =	"Math. Ann.",
	volume =	"138",
	year =		"1959",
	pages =		"1-26"
}

@article{huber:selbergII,
	author =	"Heinz Huber",
	title =	"Zur analytischen {T}heorie hyperbolischer {R}aumformen und {B}ewegungsgruppen, {II}",
	journal =	"Math. Ann.",
	volume =	"142",
	year =		"1961",
	pages =		"385-398"
}

@article{huber:selbergIIA,
	author =	"Heinz Huber",
	title =	"Zur analytischen {T}heorie hyperbolischer {R}aumformen und {B}ewegungsgruppen, {II}:  {N}achtrag",
	journal =	"Math. Ann.",
	volume =	"143",
	year =		"1961",
	pages =		"463-464"
}

@article{mr:flat,
    title = {{Length spectra and $p$-spectra of compact flat manifolds}},
    author = {Roberto J. Miatello and Juan Pablo Rossetti},
	journal =	"J. Geom. Analysis",
volume="13",
pages="631-657",
year="2003",
    eprint = {arXiv:math.DG/0110325}
}

@article{mr:p,
    title={{Flat manifolds isospectral on $p$-forms}},
    author = {Roberto J. Miatello and Juan Pablo Rossetti},
	journal =	"J. Geom. Analysis",
	volume =	"11",
	year =		"2001",
	pages =		"647-665",
    eprint = {arXiv:math.DG/0303276}

}

@article{selberg:selberg,
	author =	"Atle Selberg",
	title =		"Harmonic analysis and discontinuous groups in weakly symmetric Riemannian spaces with applications to Dirichlet series",
	journal =	"J. Indian Math. Soc. (N.S.)",
	volume =	"20",
	year =		"1956",
	pages =		"47-87"
}
@article{sunada:flat,
	author =	"Toshikazu Sunada",
	title =		"Spectrum of a compact flat manifold",
	journal =	"Comment. Math. Helv",
	volume =	"53",
	year =		"1978",
	pages =		"613-621"
}

@article{conwaysloane:four,
        author =        "John Horton Conway and Neil J. A. Sloane",
        title =         "Four-dimensional lattices with the same theta series",
        journal =       "IMRN",
        volume =        "4",
        year =          "1992",
        pages =         "93-96"
}

@article{schiemann:three,
        author =        "Schiemann, Alexander",
        title =         "Ternary positive definite quadratic forms are determined by their theta series",
        journal =       "Math. Ann.",
        volume =        "308",
        year =          "1997",
        pages =         "507-517"
}


@article{milnor:sixteen,
        author =        "John Milnor",
        title =         "Eigenvalues of the {L}aplace operator on certain manifolds",
        journal =       "Proc. Nat. Acad. Sci. USA",
        volume =        "51",
        year =          "1964",
        pages =         "542"
}

@article{gordon:survey,
        author =        "Carolyn S. Gordon",
        title =         "Isospectral manifolds with different local geometry",
        journal =       "J. Korean Math. Soc.",
        volume =        "38",
        year =          "2001",
        pages =         "955-970"
}

@book{chavel:eigen,
	author =		"Isaac Chavel",
	title =	"Eigenvalues in Riemannian Geometry",
	publisher =	"Academic Press",
	year =		"1984"
}

@article{phillipssarnak:PGT,
author = "Ralph Phillips and Peter Sarnak",
title = "Geodesics in homology classes",
journal = "Duke Math. J.",
volume = "55",
year = "1987",
pages = "287-297"
}

@inproceedings{conway:orbifold,
	author ="John Horton Conway",
	title  ="The orbifold notation for surface groups",
	booktitle ="Groups, Combinatorics and Geometry",
	publisher="Cambridge University Press",
	pages="438-447",
	year =	"1992"}



@article{sunada:method,
author="T. Sunada",
title="Riemannian coverings and isospectral manifolds",
journal="Annals of Math.",
volume="121",
year="1985",
pages="169-186"
}

@article{vigneras:isospectral,
author="M.-F. Vigneras",
title="Variet\'es Riemanniennes isospectrales et non isom\'etriques",
journal="Annals of Math.",
volume="112",
year="1980",
pages="21-32"
}

@book{buser:book,
author="Peter Buser",
title="Geometry and Spectra of Compact Riemann Surfaces",
publisher="Birkh{\"a}user",
year="1992"
}

@misc{doylerossetti:surfaces,
title = {{Isospectral hyperbolic surfaces have matching geodesics}},
author = {Peter G. Doyle and Juan Pablo Rossetti},
eprint = {arXiv:math.DG/0605765}}

